Locating Charging Stations: Connected, Capacitated and Prize- Collecting

In this paper, we study locating charging station problem as facility location problem and its variants ($k$-Median, $k$-Facility location and $k$-center). We study the connectivity and the capacity constraints in these problem. Capacity and connectivity constraints have been studied in the literature separately for all these problems. We give first constant factor approximations when both the constraints are present. Extending/modifying the techniques used for connected variants of the problem to include capacities or for capacitated variants of problem to include connectivity is a tedious and challenging task. In this paper, we combine the two constraints by reducing the problem to underlying well studied problems, solving them as black box and combine the obtained solutions. We also, combine the two constraints in the prize-collection set up. In the prize-collecting set up, the problems are not even studied when one of the constraint is present. We present constant factor approximation for them as well.

==> CPFL_copy_for_journal.tex <==
\section{Solving ConPFL via reduction to ConFL}
\label{sectionConPFL}
In this section, we will be presenting a constant factor approximation for ConPFL using LP rounding techniques and reduction to ConFL.

ConPFL can be formulated as following integer program:

\label{{ConPFL}}
$\text{Minimise} ~Cost(w,x,y,z) = \sum_{i \in \facilityset} w_iy_i + \sum_{i \in \facilityset}\sum_{j \in \cliset} \dist{i}{j}x_{ij} + \sum_{e \in \edgeset} \concost{e} y_e + \sum_{j \in \cliset} p_j z_j $
\begin{eqnarray}
\text{subject to} &  \sum_{i \in \facilityset} x_{ij} + z_j = 1 ~ &\forall j \in \cliset \label{const1}\\ 
&  x_{ij} \leq w_i~& \forall i \in \facilityset,~\forall j \in \cliset \label{const2}\\ 
&  w_v = 1 \label{const3}\\   
&  \sum_{i \in S} x_{ij} \leq \sum_{e \in \delta(S)}y_e~& \forall S \subseteq \facilityset,~v\notin S~\forall j \in \cliset \label{const4}\\   
& w_i, x_{ij}, y_e, z_j \in \left\lbrace 0,1 \right\rbrace  ~&\forall~i \in \facilityset,~\forall j \in \cliset,~\forall e \in \edgeset \label{const5}
\end{eqnarray}

where variable $w_i$ denotes whether facility $i$ is open or not, $x_{ij}$ indicates if client $j$ is served by facility $i$ or not, $y_e$ denoted whether edge $e$ belongs to steiner tree or not and $z_j$ denotes if client $j$ pay penalty or not. Constraints~\ref{const1} ensures that every client ensures that every client is either served or pays penalty. Constraints~\ref{const2} ensures that a client is assigned to a open facility only. Constraint~\ref{const3} ensures that the facility $v$ is opened. \textcolor{red}{Need to talk about guess of v somewhere..} Constraints~\ref{const4} ensures...\textcolor{red}{have to explain delta(S) and connectivity here.. } LP-Relaxation of the problem is obtained by allowing the variables $ w_i, x_{ij}, y_e, z_j \in [0, 1]$. Let $\rho^{*} = <w^*,x^*, y^*, z^*>$ denote the optimal solution of the LP and $\Opt{\conpfl}$ denote the cost of $\rho^*$.

\subsection{Identifying the Clients that will Pay Penalty ($\cliset'$)}
We first identify a set of clients $\cliset'$ that will be paying penalty in our solution $AS_{\conpfl}$. Once we have identified these clients, we will handle the remaining clients separately. The idea is to select clients that are not served to a large extent in LP solution or in other words, the clients that were paying penalty to a large extent (say $\geq 1/2$). Formally, for every client $j$ such that $z^*_j \geq 1/2$: add $j$ to $\cliset'$, set $z'_j=1$ and $x'_{ij}=0$ for every $i$. Note that, this can be done within $2$ factor of penalty cost, that is, $\sum_{j \in \cliset'}p_jz'_j \leq 2 \sum_{j \in \cliset'}p_j z^*_j$. 

\subsection{An instance $I_{\confl}$ of \ConFL
}
Next, we create an instance $I_{\confl}$ of ConFL wherein the client set is reduced to $\cliset \setminus \clientset'$. The following lemma shows existence of a feasible fractional solution to $I_{\confl}$ such that the cost is bounded within a constant factor of LP optimal ($\Opt{\conpfl}$). 

\begin{lemma}
\label{fs_confl}
There exist a fractional feasible solution $\rho' = <w', x', y'>$ such that  $Cost(\rho') \leq 2(\sum_{i \in \facilityset} f_iw^*_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e)$.
\end{lemma}

\begin{proof}

Recall that, every client $j \in \cliset \setminus \cliset'$ is served to an extent of at least $1/2$. For all $i \in \facilityset : x^*_{ij}> 0 $, we raise the assignment of $j$ on $i$ proportionately so that $j$ is fully served. Variables $w$ and $y$ are raised accordingly to satisfy constraints~(\ref{const2}) and constraints~(\ref{const4}) respectively. Formally, $\forall j \in \cliset \setminus \cliset'$, $\forall i \in \facilityset$ and $\forall e \in \edgeset$, set $(i)$ ${x}'_{ij} = x^*_{ij}/\sum_{i \in \facilityset}x^*_{ij}$, $(ii)$ $w'_i  = \min \{1, w^*_i \cdot \max_{j \in \cliset \setminus \cliset' : x^*_{ij} > 0 } \{{x}'_{ij}/x^*_{ij} \}\}$ and $(iii)$ $y'_e = \max \{ 1, 2y^*_e \}$. 

Next, we will see that $\rho'<w', x', y'>$ is a feasible solution to LP of ConFL:

\label{{ConFL}}
$\text{Minimise} ~Cost(w,x,y) = \sum_{i \in \facilityset} w_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x_{ij} + \sum_{e \in \edgeset} \concost{e} y_e $
\begin{eqnarray}
\text{subject to} &  \sum_{i \in \facilityset} x_{ij} = 1 ~ &\forall j \in \clientset \setminus \clientset' \label{LP2_const1}\\ 
&  x_{ij} \leq w_i~& \forall i \in \facilityset,~\forall j \in \clientset \setminus \clientset' \label{LP2_const2}\\ 
&  w_v = 1 \label{LP2_const3}\\   
&  \sum_{i \in S} x_{ij} \leq \sum_{e \in \delta(S)}y_e~& \forall S \subseteq \facilityset,~v\notin S~\forall j \in \cliset \setminus \clientset' \label{LP2_const4}\\   
& 0 \leq w_i, x_{ij}, y_e \leq 1   ~&\forall~i \in \facilityset,~\forall j \in \clientset \setminus \clientset',~\forall e \in \edgeset \label{const5}
\end{eqnarray}

\begin{enumerate}
    \item Constraints~\ref{LP2_const1} are satisfied because for all $j \in \clientset \setminus \clientset'$, $\sum_{i \in \facilityset} x'_{ij} = \sum_{i \in \facilityset} (x^*_{ij}/\sum_{i \in \facilityset}x^*_{ij}) = 1$.
    \item Constraint~\ref{LP2_const2} is satisfied because $w'_v = w^*_v = 1$.
    \item Constraints~\ref{LP2_const3} holds trivially if $w'_i = 1$ as $x'_{ij} \leq 1$. Otherwise, for $x^*_{ij} > 0$, $w'_i \geq (w^*_i/x^*_{ij}) x'_{ij} \geq x'_{ij}$ as $w^*_i/x^*_{ij} \geq 1$
    \item For $y'_e = 1$, constraints~\ref{LP2_const4} holds because $\sum_{i \in S} x'_{ij} \leq 1$. Otherwise, $\sum_{e \in \delta(S)}y'_e = \frac{\sum_{e \in \delta(S)} y^*_2}{2} \geq \frac{\sum_{i \in S} x^*_{ij}}{2} \geq \frac{\sum_{i \in S} x^*_{ij}}{\sum_{i \in \facilityset} x^*_{ij}} = \sum_{i \in S}x'_{ij}$ where the last inequality follows because $\sum_{i \in \facilityset}x^*_{ij} \geq 1/2$ for all $j \in \clientset \setminus \clientset'$.
\end{enumerate}

\textbf{Cost Bound:} Next we will bound the cost of our feasible solution $\rho'$. Note that, ($i$) $x'_{ij} = x^*_{ij}/\sum_{i \in \facilityset} x^*_{ij} \leq 2 x^*_{ij}$, $(ii)$ $w'_i \leq 2 w^*_i$ and ($iii$) $y'_e \leq 2 y^*_e$. Therefore, $Cost(\rho') = Cost(w',x',y') = \sum_{i \in \facilityset} w'_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x'_{ij} + \sum_{e \in \edgeset} \concost{e} y'_e  \leq 2 ( \sum_{i \in \facilityset} w^*_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e)$.
\end{proof}

Next, we solve the instance $I_{\confl}$ using the approximation algorithm of Gupta~\etal~\cite{ConFLGupta2001} as black-box to obtain an approximate solution $AS_{\confl}$. Their algorithm can be used because they use LP rounding techniques wherein they first solve the LP of \ConFL for which we have provided a feasible solution in Lemma~\ref{fs_confl}. Note that, we can not use other (better) approximation algorithms as black-box because the feasible solution we have provided may not be integral, in fact most of the times it is not. The solution $AS_{\confl}$ along with clients in $\clientset'$ forms an approximate solution $AS_{\conpfl}$ for ConPFL. The final cost bound is as follows: $ Cost(AS_{\conpfl}) = Cost(AS_{\confl}) + \sum_{j \in \clientset'} p_j z'_j \leq \beta Cost(\Opt{\confl}) + 2 \sum_{j \in \clientset'} p_j z^*_j  \leq \beta Cost(\rho') + 2 \sum_{j \in \clientset'} p_j z^*_j \leq 2 \beta (\sum_{i \in \facilityset} w^*_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e) + 2 \sum_{j \in \clientset'} p_j z^*_j \leq 2 \beta Cost(\rho^*) = 2 \beta Cost(\Opt{\conpfl})$ where the first inequality follows for $\beta$-factor approximation of \ConFL and second and third inequality follows from Lemma~\ref{fs_confl}. Using Gupta~\etal~\cite{ConFLGupta2001}, we have $\beta=10.66$ which gives us $21.32$-factor approximation.

==> ConPFL_copy_for_journal.tex <==
\section{Solving ConPFL via reduction to ConFL}
\label{sectionConPFL}
In this section, we will be presenting a constant factor approximation for ConPFL using LP rounding techniques and reduction to ConFL.

ConPFL can be formulated as following integer program:

\label{{ConPFL}}
$\text{Minimise} ~Cost(w,x,y,z) = \sum_{i \in \facilityset} w_iy_i + \sum_{i \in \facilityset}\sum_{j \in \cliset} \dist{i}{j}x_{ij} + \sum_{e \in \edgeset} \concost{e} y_e + \sum_{j \in \cliset} p_j z_j $
\begin{eqnarray}
\text{subject to} &  \sum_{i \in \facilityset} x_{ij} + z_j = 1 ~ &\forall j \in \cliset \label{const1}\\ 
&  x_{ij} \leq w_i~& \forall i \in \facilityset,~\forall j \in \cliset \label{const2}\\ 
&  w_v = 1 \label{const3}\\   
&  \sum_{i \in S} x_{ij} \leq \sum_{e \in \delta(S)}y_e~& \forall S \subseteq \facilityset,~v\notin S~\forall j \in \cliset \label{const4}\\   
& w_i, x_{ij}, y_e, z_j \in \left\lbrace 0,1 \right\rbrace  ~&\forall~i \in \facilityset,~\forall j \in \cliset,~\forall e \in \edgeset \label{const5}
\end{eqnarray}

where variable $w_i$ denotes whether facility $i$ is open or not, $x_{ij}$ indicates if client $j$ is served by facility $i$ or not, $y_e$ denoted whether edge $e$ belongs to steiner tree or not and $z_j$ denotes if client $j$ pay penalty or not. Constraints~\ref{const1} ensures that every client ensures that every client is either served or pays penalty. Constraints~\ref{const2} ensures that a client is assigned to a open facility only. Constraint~\ref{const3} ensures that the facility $v$ is opened. \textcolor{red}{Need to talk about guess of v somewhere..} Constraints~\ref{const4} ensures...\textcolor{red}{have to explain delta(S) and connectivity here.. } LP-Relaxation of the problem is obtained by allowing the variables $ w_i, x_{ij}, y_e, z_j \in [0, 1]$. Let $\rho^{*} = <w^*,x^*, y^*, z^*>$ denote the optimal solution of the LP and $\Opt{\conpfl}$ denote the cost of $\rho^*$.

\subsection{Identifying the Clients that will Pay Penalty ($\cliset'$)}
We first identify a set of clients $\cliset'$ that will be paying penalty in our solution $AS_{\conpfl}$. Once we have identified these clients, we will handle the remaining clients separately. The idea is to select clients that are not served to a large extent in LP solution or in other words, the clients that were paying penalty to a large extent (say $\geq 1/2$). Formally, for every client $j$ such that $z^*_j \geq 1/2$: add $j$ to $\cliset'$, set $z'_j=1$ and $x'_{ij}=0$ for every $i$. Note that, this can be done within $2$ factor of penalty cost, that is, $\sum_{j \in \cliset'}p_jz'_j \leq 2 \sum_{j \in \cliset'}p_j z^*_j$. 

\subsection{An instance $I_{\confl}$ of \ConFL
}
Next, we create an instance $I_{\confl}$ of ConFL wherein the client set is reduced to $\cliset \setminus \clientset'$. The following lemma shows existence of a feasible fractional solution to $I_{\confl}$ such that the cost is bounded within a constant factor of LP optimal ($\Opt{\conpfl}$). 

\begin{lemma}
\label{fs_confl}
There exist a fractional feasible solution $\rho' = <w', x', y'>$ such that  $Cost(\rho') \leq 2(\sum_{i \in \facilityset} f_iw^*_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e)$.
\end{lemma}

\begin{proof}

Recall that, every client $j \in \cliset \setminus \cliset'$ is served to an extent of at least $1/2$. For all $i \in \facilityset : x^*_{ij}> 0 $, we raise the assignment of $j$ on $i$ proportionately so that $j$ is fully served. Variables $w$ and $y$ are raised accordingly to satisfy constraints~(\ref{const2}) and constraints~(\ref{const4}) respectively. Formally, $\forall j \in \cliset \setminus \cliset'$, $\forall i \in \facilityset$ and $\forall e \in \edgeset$, set $(i)$ ${x}'_{ij} = x^*_{ij}/\sum_{i \in \facilityset}x^*_{ij}$, $(ii)$ $w'_i  = \min \{1, w^*_i \cdot \max_{j \in \cliset \setminus \cliset' : x^*_{ij} > 0 } \{{x}'_{ij}/x^*_{ij} \}\}$ and $(iii)$ $y'_e = \max \{ 1, 2y^*_e \}$. 

Next, we will see that $\rho'<w', x', y'>$ is a feasible solution to LP of ConFL:

\label{{ConFL}}
$\text{Minimise} ~Cost(w,x,y) = \sum_{i \in \facilityset} w_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x_{ij} + \sum_{e \in \edgeset} \concost{e} y_e $
\begin{eqnarray}
\text{subject to} &  \sum_{i \in \facilityset} x_{ij} = 1 ~ &\forall j \in \clientset \setminus \clientset' \label{LP2_const1}\\ 
&  x_{ij} \leq w_i~& \forall i \in \facilityset,~\forall j \in \clientset \setminus \clientset' \label{LP2_const2}\\ 
&  w_v = 1 \label{LP2_const3}\\   
&  \sum_{i \in S} x_{ij} \leq \sum_{e \in \delta(S)}y_e~& \forall S \subseteq \facilityset,~v\notin S~\forall j \in \cliset \setminus \clientset' \label{LP2_const4}\\   
& 0 \leq w_i, x_{ij}, y_e \leq 1   ~&\forall~i \in \facilityset,~\forall j \in \clientset \setminus \clientset',~\forall e \in \edgeset \label{const5}
\end{eqnarray}

\begin{enumerate}
    \item Constraints~\ref{LP2_const1} are satisfied because for all $j \in \clientset \setminus \clientset'$, $\sum_{i \in \facilityset} x'_{ij} = \sum_{i \in \facilityset} (x^*_{ij}/\sum_{i \in \facilityset}x^*_{ij}) = 1$.
    \item Constraint~\ref{LP2_const2} is satisfied because $w'_v = w^*_v = 1$.
    \item Constraints~\ref{LP2_const3} holds trivially if $w'_i = 1$ as $x'_{ij} \leq 1$. Otherwise, for $x^*_{ij} > 0$, $w'_i \geq (w^*_i/x^*_{ij}) x'_{ij} \geq x'_{ij}$ as $w^*_i/x^*_{ij} \geq 1$
    \item For $y'_e = 1$, constraints~\ref{LP2_const4} holds because $\sum_{i \in S} x'_{ij} \leq 1$. Otherwise, $\sum_{e \in \delta(S)}y'_e = \frac{\sum_{e \in \delta(S)} y^*_2}{2} \geq \frac{\sum_{i \in S} x^*_{ij}}{2} \geq \frac{\sum_{i \in S} x^*_{ij}}{\sum_{i \in \facilityset} x^*_{ij}} = \sum_{i \in S}x'_{ij}$ where the last inequality follows because $\sum_{i \in \facilityset}x^*_{ij} \geq 1/2$ for all $j \in \clientset \setminus \clientset'$.
\end{enumerate}

\textbf{Cost Bound:} Next we will bound the cost of our feasible solution $\rho'$. Note that, ($i$) $x'_{ij} = x^*_{ij}/\sum_{i \in \facilityset} x^*_{ij} \leq 2 x^*_{ij}$, $(ii)$ $w'_i \leq 2 w^*_i$ and ($iii$) $y'_e \leq 2 y^*_e$. Therefore, $Cost(\rho') = Cost(w',x',y') = \sum_{i \in \facilityset} w'_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x'_{ij} + \sum_{e \in \edgeset} \concost{e} y'_e  \leq 2 ( \sum_{i \in \facilityset} w^*_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e)$.
\end{proof}

Next, we solve the instance $I_{\confl}$ using the approximation algorithm of Gupta~\etal~\cite{ConFLGupta2001} as black-box to obtain an approximate solution $AS_{\confl}$. Their algorithm can be used because they use LP rounding techniques wherein they first solve the LP of \ConFL for which we have provided a feasible solution in Lemma~\ref{fs_confl}. Note that, we can not use other (better) approximation algorithms as black-box because the feasible solution we have provided may not be integral, in fact most of the times it is not. The solution $AS_{\confl}$ along with clients in $\clientset'$ forms an approximate solution $AS_{\conpfl}$ for ConPFL. The final cost bound is as follows: $ Cost(AS_{\conpfl}) = Cost(AS_{\confl}) + \sum_{j \in \clientset'} p_j z'_j \leq \beta Cost(\Opt{\confl}) + 2 \sum_{j \in \clientset'} p_j z^*_j  \leq \beta Cost(\rho') + 2 \sum_{j \in \clientset'} p_j z^*_j \leq 2 \beta (\sum_{i \in \facilityset} w^*_iy_i + \sum_{i \in \facilityset}\sum_{j \in \clientset \setminus \clientset'} \dist{i}{j}x^*_{ij} + \sum_{e \in \edgeset} \concost{e} y^*_e) + 2 \sum_{j \in \clientset'} p_j z^*_j \leq 2 \beta Cost(\rho^*) = 2 \beta Cost(\Opt{\conpfl})$ where the first inequality follows for $\beta$-factor approximation of \ConFL and second and third inequality follows from Lemma~\ref{fs_confl}. Using Gupta~\etal~\cite{ConFLGupta2001}, we have $\beta=10.66$ which gives us $21.32$-factor approximation.

==> Intro_new.tex <==
\section{Introduction}

\begin{figure}
    \centering
    \includegraphics[width=10cm]{Figures/f5.png}
    \caption{Combining connectivity and capacities. Using ConFL instead of Con$k$M and Con$k$FL as black-box in ($c$) and ($d$) will also work and will reduce the cost of solution.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=7cm]{Figures/f6.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


{\em Facility Location Problem} (FL) and $k$-Median ($k$M) are well known and well studied problem in operations research and computer science~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,guha1999greedy,KPR,Chudak98,mahdian2001greedy,mahdian_1.52,charikar2005improved,arya,Zhang2007126,Li13}. In (uncapacitated) FL, we are given a set $\facilityset$ of facilities and a set $\cliset$ of clients.  A facility $i$ in $\facilityset$ has an associated {\em facility opening cost} $f_i$. $\dist{i}{j}$ denotes the cost of serving client $j$ from a facility $i$. We assume that the service cost is a metric.
%The distances between client $j$ and facility $i$, denoted by $\dist{i}{j}$ forms a metric.
The goal is to open $\facilityset' \subseteq \facilityset$ so as to minimise the sum of facility opening costs ({\em facility cost}) and the total {\em service cost} of serving all the clients from the opened facilities. 
%which is defined to be sum of distances from each client to the opened facility it is getting served from.
%Whereas 
In (uncapacitated) $k$M, we are given an upper bound $k$ ({\em cardinality constraint}) on the maximum number of facilities that can be opened in our solution and facility opening costs are $0$ for every facility. $k$-Facility Location is a common generalisation of FL and $k$M where in we have both the facility opening costs and the cardinality constraint.
In some applications, there is an upper bound $u_i$ on the number of clients an opened facility $i$ can serve. We call these upper bounds as capacities and the respective problems are called, {\em Capacitated Facility Location Problem} (CFL), Capacitated $k$-Median Problem (C$k$M) and Capacitated $k$-Facility Location Problem (C$k$FL).
\textcolor{red}{Do we need uniform anywhere?} The capacities are called uniform if $u_i$ is same for all $i$ in $\facilityset$.
\textcolor{red}{ If we are dealing with non-uniform then we don't need to say it explicitly...that is default....SO delete...
We will be dealing with general/non-uniform capacities in this paper.}

In some applications, it is important for the opened facilities to be connected to each other. For example, consider a telecommunication network model with a {\em central core} consisting of interconnected nodes and there is a set of {\em end nodes} that want to communicate with each other. Each core node (facility) has a switch cost and connecting central nodes to each other incurs some connection cost.  The goal is to select a subset of core nodes, connect these nodes to each other and end nodes (clients) to one of the selected core nodes so as to design a network of minimum cost. Such a variant of FL is called {\em Connected Facility Location Problem} (ConFL). ConFL is same as FL except we are also given distance $\concost{e}$ for every edge $e=(i_1, i_2)$ where $i_1,i_2 \in \facilityset$. %In a telecommunication network, the parameter $M$ reflects per unit cost of connection. 
The connectivity of the opened facilities is captured by a {\em Steiner tree} $T$, i.e., a tree connecting opened facilities but may consist of non-facility (client) nodes. %The total cost of interconnecting the facilities is $M$ times the cost of the steiner tree $T$. 
We call this cost the {\em connection cost}. We aim to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and the connection cost. ConFL is studied in the literature~\cite{ConFLGupta2001, ConFLGupta2004, ConFLSwamy2004,ConFLChwa2009,ConFLEisenbrand2010,ConFLGrandoni2011} and the current best approximation is due to Grandoni and Rothvob~\cite{ConFLGrandoni2011}. They used sampling techniques to give a $3.19$-factor approximation for the problem. Similar to CFL, variants of ConFL where we have cardinlity constraint have been studied in the literature, namely {\em Connected $k$-Median Problem} (\ConkM) and {\em Connected $k$-Facility Location Problem} (\ConkFL). The current best factor approximations ($6.98$) for \ConkM and \ConkFL are due to Eisenbrand~\etal~\cite{ConFLEisenbrand2010}.

\textcolor{red}{Though FL/$k$M/$k$FL have been studied with capacities and connectivity separately, to the best of our knowledge, their common generalisations where in we have both connectivity and the capacity constraints have not been studied earlier.  We call these variants, {\em Connected Capacitated Facility Location Problem} (\ConCFL), {\em Connected Capacitated $k$-Median Problem} (\ConCkM) and, {\em Connected Capacitated Facility Location Problem} (\ConCkFL) respectively.  Applications of these generalisations can be found in real life. In our example of telecommunication networks, as the switches have a limited number of slots, there is a natural cap on the maximum number of end nodes that can be connected to a core node. In this paper, we present \textcolor{blue}{first}
constant factor approximations for the problems by combining the solutions of the capacitated variants of the underlying problems (\CFL, \CkM, \CkFL) and \ConFL .
The violations in capacities/cardinality, if any, in the solutions of the underlying problems, are preserved. For \ConCkM and \ConCkFL, we present first approximations and for \ConCFL, our result is the first true approximation. To the best of our knowledge, the only result known for ConCFL is by Friggstad~\etal~\cite{FriggstadConLUFL2016}. They gave a constant factor approximation for lower and (uniform) upper bounded ConFL violating both the upper as well as the lower bounds.
{We cannot get rid of the  violations in the upper bounds even when there are no lower bounds using their technique as they use LP rounding and the LP is known to have an unbounded integrality gap.}
In this paper, we give the first true constant $(13.19)$-factor approximation for the problem using a true approximation for the CFL problem. In particular, we present the following: 
 }

Thought FL and its variants have been studied with capacities and connectivity separately, to the best of our knowledge, the common generalisations of FL/$k$M/$k$FL, where we have both connectivity and the capacity constraints have not been studied in the literature. We call these variants, {\em Connected Capacitated Facility Location Problem} (\ConCFL), {\em Connected Capacitated $k$-Median Problem} (\ConCkM) and, {\em Connected Capacitated Facility Location Problem} (\ConCkFL) respectively. The problems are same as \ConFL/\ConkM/\ConkFL except every facility $i$ can serve at most $u_i$ number of clients. \textcolor{red}{In this paper, we present \textcolor{blue}{first}
constant factor approximations for the problems by combining the solutions of the underlying problems (\CFL, \CkM, \CkFL) and \ConFL .
\textcolor{blue}{
The violations in capacities/cardinality, if any, in the solutions of the underlying problems, are preserved. For \ConCkM and \ConCkFL, we present first approximations and for \ConCFL, our result is the first true approximation.}
While combining the solutions, the violation in capacities/cardinality are preserved from the underlying problems}.
\st{
We first present our technique for \ConCFL by combining the solutions of \CFL and \ConFL and then extend these results to other variants.} To the best of our knowledge, the only known result for ConCFL in the literature is by Friggstad~\etal~\cite{FriggstadConLUFL2016}. They gave a constant factor approximation for lower and (uniform) upper bounded ConFL violating both upper and lower bounds.% A constant factor approximation for ConCFL with constant factor violation in capacities when the capacities are uniform follows as a special case of their problem. 
\st{
Firstly, their result holds only for uniform capacities.
Secondly, they violate the capacities.}
\textcolor{blue}{We cannot get rid of the  violations in the upper bounds even when there are no lower bounds using their technique as they use LP rounding and the LP is known to have an unbounded integrality gap.}
Their result can not be extended to get rid of violation in upper bounds even when there are no lower bounds as they use LP rounding techniques and the LP is known to have an unbounded integrality gap. % Finally, their factor is dependent on.... which can be large for small violation in capacities. 
In this paper, we give the first true constant $(13.19)$-factor approximation for the problem with non-uniform capacities. In particular, we present the following: 

\begin{theorem}
\label{thm_ConCFL}
Given an $\alpha$-factor approximation for \CFL/\CkM/\CkFL with $\gamma$-factor violation in capacity/cardinality and a $\beta$-factor approximation for \ConFL, 
a $(2\alpha+\beta)$-factor approximation for \ConCFL/\ConCkM/\ConCkFL with $\gamma$-factor violation in capacity/cardinality respectively can be obtained in polynomial time.
\end{theorem}

%The technique presented in our paper is very flexible as our factor can be improved without any change in the algorithm if, in future, the factors of the underlying problems improve. Also, the ideas extends easily to other variants of the problems. We get similar results for \ConCkM and \ConCkFL as mentioned in Theorem~\ref{thm_ConkM} and Theorem~\ref{thm_ConCkFL} respectively. To the best of our knowledge, these are the first approximations for the problems.

%\begin{theorem}
%\label{thm_ConkM}
%Given an $\alpha$-factor approximation for \CkM with $\gamma$ factor violation in capacities and a $\beta$-factor approximation for \ConFL, a $(2\alpha+\beta)$-factor approximation for \ConCkM with $\gamma$-factor violation in capacities can be obtained in polynomial time.
%\end{theorem}

%\begin{theorem}
%\label{thm_ConCkFL}
%Given an $\alpha$-factor approximation for \CkFL with $\gamma$ factor violation in capacities and a $\beta$-factor approximation for \ConFL, a $(2\alpha+\beta)$-factor approximation for \ConCkFL with $\gamma$-factor violation in capacities by $\gamma$-factor can be obtained in polynomial time.
%\end{theorem}

\textcolor{red}{ I am here..ng...are we not studying PkM and PkFL?
We next consider another variant of facility location problem, called {\em Connected Prize-Collection Facility Location} (\ConPFL). In the above formulations of the problem (say in telecommunication network), a few distant clients can affect the cost of the solution disproportionately. {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. \PFL is a well studied problem in the literature~\cite{charikar2001algorithms, jain2003greedy, Wang2015penalties, xu2005lp, xu2009improved, LiDXX15, QiuWalter}. We study the connected variant of \PFL. The two underlying problems here are \PFL and \ConFL and it is tempting to use combination of the two problems to obtain the solution. However, the combination technique does not extend to this variant of the problem because it is difficult to reduce \ConPFL to \ConFL directly within constant cost bounds. To handle this problem, we take help from LP-rounding techniques. We present the first constant ($21.31$)-factor approximation for the problem by using LP rounding technique followed by reduction to \ConFL.  In particular, we present the following:}



We next study another variant of connected facility location problem, called {\em Connected Prize-Collection Facility Location} (\ConPFL). In the above formulations of the problem (say in telecommunication network), a few distant clients can affect the cost of the solution disproportionately. {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. \PFL is a well studied problem in the literature~\cite{charikar2001algorithms, jain2003greedy, Wang2015penalties, xu2005lp, xu2009improved, LiDXX15, QiuWalter}. We study the connected variant of \PFL. The two underlying problems here are \PFL and \ConFL and it is tempting to use combination of the two problems to obtain the solution. However, the combination technique does not extend to this variant of the problem because it is difficult to reduce \ConPFL to \ConFL directly within constant cost bounds. To handle this problem, we take help from LP-rounding techniques. We present the first constant ($21.31$)-factor approximation for the problem by using LP rounding technique followed by reduction to \ConFL.  In particular, we present the following:

\begin{theorem}
\label{thm_ConPFL}
Given a $\beta$-factor approximation for \ConFL (obtained using LP rounding techniques), a $2\beta$-factor approximation for \ConPFL can be obatined in polynomial time.
\end{theorem}


Finally, we consider the most common generalisation of the problems studied in the paper, that is, we combine capacities, connectivity and penalties in facility location problem. We call the problem as {\em Connected Capacitated Prize-Collecting Facility Location Problem} (\ConCPFL). We extend the ideas of combination technique to present the first constant ($31.31$) factor approximation for the problem with general capacities. The two underlying problems considered are {Capacitated Prize-Collecting Facility Location Problem} (\CPFL) and  {Connected Prize-Collecting Facility Location Problem} (\ConPFL). The idea extends to the problem with cardinality constraint as well, that is, to {\em Connected Capacitated Prize-Collecting $k$-Facility Location Problem}(\ConCPkFL).  In particular, we present the following:

\begin{theorem}
\label{thm_ConCPFL}
Given an $\alpha$-factor approximation for \CPFL/\CPkFL with $\gamma$-factor violation in capacities and a $\beta$-factor approximation for \ConPFL, 
a $(2\alpha+\beta)$-approximation for \ConCPFL/\ConCPkFL with $\gamma$-factor violation in capacities can be obtained in polynomial time.
\end{theorem}

Table~\ref{tab_results1}, ~\ref{tab_results2} and ~\ref{tab_results3} summarises the results of this paper. 

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 1 (Factor, Violation)}  &\textbf{ Factor} & \textbf{Violation} \\ 
         \hline
         (U)\ConCFL  & (U)\CFL ($3$, Nil) ~\cite{Aggarwal}  & $9.19$ & Nil \\
         \hline
         (NU)\ConCFL  & (NU)\CFL($5$, Nil) ~\cite{Bansal} &  $13.19$ & Nil \\
         \hline
         (U)\ConCkM & (U)\CkM($ O(1/\epsilon),(1+\epsilon)u$)~\cite{ByrkaRybicki2015} &  $O(1/\epsilon)$  & $(1+\epsilon)u$ \\
         \hline 
         (NU)\ConCkM & (NU)\CkM($ O(1/\epsilon) ,(1+\epsilon)u$)~\cite{Demirci2016} &  $O(1/\epsilon)$  & $(1+\epsilon)u_i$ \\
         \hline 
         (U)\ConCkFL & (U)\CkFL($O(1/\epsilon^2), (2+\epsilon)u)$~\cite{capkmByrkaFRS2013}
          & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
    \end{tabular}
    \caption{Approximations for variants of FL with connectivity and capacity. Sub-Problem 2 considered is \ConFL for which we use $3.19$-factor approximation of~\cite{ConFLGrandoni2011}). (U-Uniform, NU-Non-Uniform) }
    \label{tab_results1}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem(Factor)}  &\textbf{ Factor}  \\ 
         \hline
         \ConPFL & \ConFL (10.66) ~\cite{ConFLGupta2001} & $21.32$ \\
         \hline
  \end{tabular}
    \caption{Approximations for variant of FL with connectivity and penalty.}
    \label{tab_results2}
\end{table}  

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 1 (Factor, Violation)}  &\textbf{ Factor} & \textbf{Violation} \\ 
         \hline
         (U)\ConCPFL & (U)\CPFL($3$, Nil)~\cite{GuptaG14}) &  $27.32$ & Nil \\
         \hline
         (NU)\ConCPFL & (NU)\CPFL($5$, Nil)~\cite{GuptaG14} &  $31.32$ & Nil \\
         \hline
         (U)\ConCPkFL & (U)\CPkFL($O(1/\epsilon^2),(2+\epsilon)u$)~\cite{DabasCFLPO}) &  $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
    \end{tabular}
    \caption{Approximations for variants of FL with capacity, connectivity and penalty. Sub-Problem 2 considered is \ConPFL for which we use $21.32$-factor approximation given in this paper. (U-Uniform, NU-Non-Uniform) }
    \label{tab_results3}
\end{table}



\subsection{Additional Results}
We present one simplified result for (non-uniform) \CPFL. Though there are results known in the literature for the problem with similar approximation guarantee ($5$-factor) by ~Gupta and Gupta~\cite{GuptaG14} using local search technique. Our result is interesting as it is much simpler and uses the underlying problem {\CFL} as black box without increasing the cost. Our factor will improve, if the factor for underlying problem (non-uniform CFL) can be improved in future. In particular, we present the following:

\begin{theorem}
\label{thm_CPFL}
Given an $\alpha$-factor approximation for (non-uniform) \CFL, an $\alpha$-factor approximation for \CPFL can be obtained in polynomial time.
\end{theorem}

==> Introduction.tex <==
\section{Introduction}
{\em Facility Location Problem} (FL) is a well known and well studied problem in operations research and computer science~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,Chudak98,Li13}. In (uncapacitated) FL, we are given a set $\facilityset$ of facilities and a set $\cliset$ of clients. The distances between client $j$ and facility $i$, denoted by $\dist{i}{j}$ forms a metric. Every facility $i$ in $\facilityset$ has an associated {\em facility opening cost} $f_i$. The goal is to open $\facilityset' \subseteq \facilityset$ so as to minimise the sum of facility costs ({\em facility cost}) and the {\em service cost}, which is defined to be sum of distances from each client to the facility it is getting served from. In the above formulation of the problem, few distant clients can affect the cost of the solution disproportionately. {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. 
%We will use Facility Location with Penalty (FLwP) and prize-collecting facility location (PFL) interchangeably in the paper. 
In real life applications, there is an upper bound $u_i$ on how many clients an opened facility $i$ can serve. We call these upper bounds as capacities and the respective problems are called, {\em Capacitated Facility Location Problem} (CFL) and {\em Capacitated Prize-Collecting Facility Location Problem} (CPFL). The capacities are called uniform if $u_i$ is same for all $i$ in $\facilityset$. All the results presented in this paper are for general/non-uniform capacities.

PFL~\cite{} and CFL~\cite{Shmoys,GroverGKP18, Anfocs2014,KPR,ChudakW99,mathp,paltree,mahdian_universal,zhangchenye,Bansal,Aggarwal} are widely studied in the literature. For CPFL, Dabas~\etal~\cite{} gives an $O(1/\epsilon)$ approximation with $(1+\epsilon)$ factor violation in capacities using LP rounding techniques and reduction to CFL. The only true approximation is due to~Bansal~\etal~\cite{}. They uses local search to obtain a $5$-factor approximation for the problem. We first present a much simpler $5$-factor approximation algorithm for the problem via reduction to  (non-uniform) CFL. Our factor will improve, if the factor for underlying problem ((non-uniform CFL) can be improved in future. In particular, we present the following:

\begin{theorem}
\label{thm_CPFL}
There is a polynomial time $\alpha$-factor approximation algorithm for Capacitated Prize-Collecting Facility Location Problem where $\alpha$ is the approximation factor for  (non-uniform) Capacitated Facility Location Problem.
\end{theorem}

In some applications, it is important for the opened facilities to be connected to each other. For example, consider a telecommunication network model with a {\em central core} consisting of interconnected nodes and there is a set of {\em end nodes} that want to communicate with each other. Each core node (facility) has a switch cost and connected central nodes to each other incurs some connection cost.  The goal is to select a subset of core nodes, connect these nodes to each other and end nodes (clients) to one of the selected core nodes so as to design a network of minimum cost. Such a variant of FL is called {\em Connected Facility Location Problem} (ConFL). ConFL is same as FL except we are also given cost $\concost{e}$ for every edge $e=(i_1, i_2)$ where $i_1,i_2 \in \facilityset$ and an integer $M$. In a telecommunication network, the parameter $M$ reflects per unit cost of connection. The connectivity of the opened facilities is captured by a {\em Steiner tree} $T$, i.e., a tree connecting opened facilities but may consist of non-facility (client) nodes. The total cost of interconnecting the facilities is $M$ times the cost of the steiner tree $T$. We call this cost the {\em connection cost}. We aim to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and the connection cost. ConFL is studied in the literature~\cite{} and the current best approximation is due to Grandoni and Rothvob~\cite{}. They used sampling techniques to give a $3.19$-factor approximation for the problem. To the best of our knowledge, the generalisation of FL, where we have both connectivity constraint and the penalty costs have not been studied in the literature. We call this variant, {\em Connected Prize-Collecting Facility Location Problem} (ConPFL). The problem is same as ConFL but now some client $j$ can be left unserved by paying penalty $p_j$. The aim is revised so as to minimize the total of facility cost, service cost, the connection cost and the penalty cost. We present the first constant ($21.31$) factor approximation for the problem using LP rounding and reduction to ConFL. In particular, we present the following:

\begin{theorem}
\label{thm_ConPFL}
There is a polynomial time $2\beta$-factor approximation for Connected Prize-Collecting Facility Location Problem where $\beta$ is an approximation for Connected Facility Location Problem obtained using LP rounding technique.
\end{theorem}

In the telecommunication network, every central node can handle only a specific amount of traffic. Therefore, it is natural to have capacities on the central nodes (facilities). Hence, we consider a common generalisation of CPFL and ConPFL called the {\em Connected Capacitated Prize-Collecting Facility Location Problem} (ConCPFL). ConCPFL is same as ConPFL except that every facility $i$ has a capacity $u_i$. Recall that, capacity $u_i$ represents the maximum number of clients an opened facility $i$ can serve. In this paper, we present the first true constant ($31.31$) factor approximation for the problem with general capacities using combinatorial techniques. We combine solutions for CPFL and ConPFL obtained in Theorem~\ref{thm_CPFL} and Theorem~\ref{thm_ConPFL} respectively to give the following: 

\begin{theorem}
\label{thm_ConCPFL}
There is a polynomial time $(2\gamma+\lambda)$-approximation for Connected Capacitated Facility Location Problem where $\gamma$ and $\lambda$ are approximation factors for Capacitated Prize-Collecting Facility Location and Connected Prize-Collecting Facility Location Problem respectively.
\end{theorem}

%We consider two more generalisations of FL where we combine the connectivity and the capacity constraints.

As a by-product of Theorem~\ref{thm_ConCPFL},
we also give the first true constant
factor approximation for {\em Connected Capacitated Facility Location Problem} (ConCFL). ConCFL is a generalisation of CFL and ConFL. To the best of our knowledge, the only known result for ConCFL in the literature is by Friggstad~\etal~\cite{}. They give a constant factor approximation for upper and lower bounded ConFL violating both upper and lower bounds. As a special case, we get a constant factor approximation for ConCFL with constant factor violation in capacities when the capacities are uniform. \textcolor{red}{We need to comment something on factor in terms of violation for friggstad}. We give a $(13.19)$-factor approximation using solutions of two underlying problems {\em viz.} CFL and ConFL. In particular, we present the following:

\begin{theorem}
\label{thm_ConCFL}
There is a polynomial time $(2\alpha+\beta)$-approximation for Connected Capacitated Facility Location Problem where $\alpha$ and $\beta$ are approximation factors for Capacitated Facility Location and Connected Facility Location Problem respectively.
\end{theorem}

==> Related_Work_copy_for_journal.tex <==

\subsection{Previous and Related Work}
\textbf{Capaciated variants of the problem (CFL, C$k$M, C$k$FL and C$k$C)}: Shmoys \etal~\cite{Shmoys} gave the first constant factor($7$) approximation when the capacities are uniform, with a capacity blow-up of $7/2$, by rounding the solution to standard LP. Grover \etal~\cite{GroverGKP18} 
reduced the capacity violation to $(1 + \epsilon)$ thereby showing that the capacity violation can be reduced to arbitrarily close to $0$ by rounding a solution to standard LP. An \etal~\cite{Anfocs2014} gave the first true constant factor(288) approximation for the problem (non-uniform), by strengthening the standard LP. Local search has been successful in dealing with capacities, several results~\cite{KPR, ChudakW99, mathp, paltree, mahdian_universal, zhangchenye} have been successfully obtained using local search with the current best being $5$-factor for non-uniform~\cite{Bansal} and $3$-factor for uniform capacities~\cite{Aggarwal}. No true approximation is known for C$k$M, till date. Constant factor approximations~\cite{Charikar,Charikar:1999,capkmshanfeili2014,ChuzhoyR05,capkmByrkaFRS2013,aardal2013,GroverGKP18} are known, that violate capacities or cardinality by a factor of $2$ or more. Strengthened LPs and dependent rounding techniques have been used to give constant factor approximation with small violations in capacities/cardinality. For uniform capacities Byrka \etal ~\cite{ByrkaRybicki2015} and for non-uniform capacities Demirci \etal~\cite{Demirci2016} gave the approximations with $(1+\epsilon)$ violation in capacities whereas Li~\cite{capkmshili2014, Lisoda2016} gave the approximations using at most  $(1 + \epsilon) k$ facilities for uniform as well as non-uniform capacities. For uniform C$k$FL, a constant factor approximation, with $(2 + \epsilon)$ violation in capacities, was given by Byrka \etal~\cite{capkmByrkaFRS2013} using dependent rounding. This was followed by two constant factor approximations by Grover \etal~\cite{GroverGKP18}, one with $(1 + \epsilon)$ violation in capacities and $2$-factor violation in cardinality and the other with $(2+\epsilon)$ factor violation in capacities only. For (uniform) C$k$C, a $10$-factor approximation was given by Bar-Ilan~\etal
~\cite{bar-IlanCkC} which was improved to $6$ by Khuller and Sussman~\cite{KhullerSussmanCkC}. For non-uniform capacities, Cygan~\etal~\cite{CyganCkC} gave a large constant factor approximation, improved to $9$ by An~\etal~\cite{AnCkC} which is also also the current best.


%Several results~\cite{Charikar,Charikar:1999,capkmshanfeili2014,KPR, capkmByrkaFRS2013} have been obtained, for C$k$M, that violate capacities by a factor of $2$ or more. For uniform capacities, Charikar \etal~\cite{Charikar:1999} gave a $16$-factor approximation  with a capacity violation bounded by a factor of 3. Byrka \etal~\cite{capkmByrkaFRS2013} and  Shanfei Li~\cite{capkmshanfeili2014}~gave constant factor approximations improving the capacity violation to $(2 + \epsilon)$.  For non - uniform capacities, Byrka \etal~\cite{capkmByrkaFRS2013} gave constant factor approximation violating the capacities by a factor of $(3 + \epsilon)$. Strengthened LPs and dependent rounding techniques have been used by Byrka \etal ~\cite{ByrkaRybicki2015} for uniform capacities and by Demirci \etal~\cite{Demirci2016} for non-uniform capacities to break the barrier of $2$ in capacity violation. Aardal \etal ~\cite{capkmGijswijtL2013} gave a $(7 + \epsilon)$ factor algorithm for non-uniform C$k$M violating the cardinality by a factor of $2$	as a special case of Capacitated $k$-FLP. Li~\cite{capkmshili2014, Lisoda2016} broke the barrier of $2$ and gave a constant factor approximation using at most  $(1 + \epsilon) k$ facilities for uniform as well as non-uniform capacities using strengthened LP called \emph{configuration LP}.  


\noindent \textbf{Connected Variants of the problem (ConFL, Con$k$M, Con$k$FL and Con$k$C):} ConFL was first introduced by Gupta~\etal~\cite{ConFLGupta2001} where they gave a $10.66$-factor approximation for the problem using LP-rounding technique. Gupta~\etal~\cite{ConFLGupta2004} described
a random facility sampling algorithm for the problem giving $9.01$-factor approximation. Primal and dual technique was first used by Swamy and Kumar~\cite{ConFLSwamy2004} to improve the factor to $8.55$ which was then improved to $6.55$ by Jung~\etal~\cite{ConFLChwa2009}. Eisenbrand~\etal~\cite{ConFLEisenbrand2010} used random sampling to improve the factor to $4$. The factor was improved to $3.19$ using similar techniques by Grandoni and Rothvob~\cite{ConFLGrandoni2011} which is also the current best for the problem. Eisenbrand~\etal~\cite{ConFLEisenbrand2010} extends their algorithm to \ConkFL giving $6.98$-factor approximation for \ConkM and \ConkFL. For Con$k$C, Ge~\etal~\cite{ge2008ConkC} gave a $3$-factor approximation when $k$ is fixed and a $6$-factor approximation for arbitrary $k$. Liang~\etal~\cite{liang2016ConkC} also gave a simpler $6$-factor approximation for the problem.

\noindent \textbf{Prize-Collecting FL (PFL)}: For PFL, a $3$-factor approximation using primal dual techniques was given by Charikar~\etal~\cite{charikar2001algorithms} which was subsequently improved to $2$ by Jain~\etal~\cite{jain2003greedy} using dual-fitting and greedy approach. Wang~\etal~\cite{Wang2015penalties} also gave a $2$-factor approximation using a combination of primal-dual and greedy technique. Later Xu and Xu~\cite{xu2005lp} gave a $2+2/e$ using LP rounding. The factor was improved  to $1.8526$ by the same authors in~\cite{xu2009improved} using a combination of primal-dual schema and local search. For linear penalties Li~\etal~\cite{LiDXX15} gave a $1.5148$-factor using LP-rounding.

\noindent \textbf{Connected and Capacitated FL (ConCFL): } A constant factor approximation for (uniform) \ConCFL with violation in capacities follows as a special case from approximation algorithm of Friggstad~\etal~\cite{FriggstadConLUFL2016} on Connected Lower and Upper Bounded Facility Location problem.

\noindent \textbf{Capacitated and Prize-Collecting variants of the problem (CPFL and CP$k$FL)}: For \CPFL, Dabas and Gupta~\cite{DabasCFLPO} gave an $O(1/\epsilon)$ approximation with $(1+\epsilon)$ factor violation in capacities using LP rounding techniques and reduction to CFL. The only true approximation is due to~Gupta and Gupta~\cite{GuptaG14}. They uses local search to obtain a $5.83$-factor and $8.532$-factor approximation for uniform and non-uniform variants respectively. For \CPkFL, Dabas and Gupta~\cite{DabasCFLPO} gave an $O(1/\epsilon^2)$-approximation algorithm with $(2+\epsilon)$-factor violation in capacities.

\noindent \textbf{ConC$k$FL, ConC$k$M, ConC$k$C, ConCPFL, ConCP$k$M, ConCP$k$FL and ConPFL}: To the best of our knowledge, no result is known for these problems in the  literature.



==> Tables.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c | cc c |cc|}
        \hline
         
         \textbf{Problem}  &  \textbf{Sub-Problem 1} & \multicolumn{2}{c|}{\textbf{Sub-Problem 2}}   &  \textbf{Factor} & \textbf{Violation}  \\ 
         
         & Factor & Factor & Violation & & \\
         
         \hline
         (U)ConCFL & ConFL~\cite{ConFLGrandoni2011} & \multicolumn{2}{c|}{(U)CFL~\cite{Aggarwal}} & & \\
          & $3.19$ & $3$ & Nil & $9.19$ & Nil \\
         \hline
         
         (NU)ConCFL  & ConFL~\cite{ConFLGrandoni2011} & \multicolumn{2}{c|}{(NU)CFL~\cite{Bansal}} & & \\
         & $3.19$ & $5$ & Nil  &  $13.19$ & Nil \\
         \hline
         
         (U)ConC$k$M & ConFL~\cite{ConFLGrandoni2011} & \multicolumn{2}{c|}{(U)C$k$M~\cite{ByrkaRybicki2015}} & & \\ 
         & $3.19$ & $ O(1/\epsilon)$ & $(1+\epsilon)u$ &  $O(1/\epsilon)$  & $(1+\epsilon)u$ \\
         \hline 
         
         (NU)ConC$k$M & ConFL~\cite{ConFLGrandoni2011} & \multicolumn{2}{c|}{(NU)C$k$M~\cite{Demirci2016}} & &\\
         & $3.19$ & $O(1/\epsilon)$ & $(1+\epsilon)u$ &  $O(1/\epsilon)$  & $(1+\epsilon)u_i$ \\
         \hline 
         
         (U)ConC$k$FL & ConFL~\cite{ConFLGrandoni2011} & \multicolumn{2}{c|}{(U)C$k$FL~\cite{capkmByrkaFRS2013}} & &\\
         & $3.19$ & $O(1/\epsilon^2)$ & $(2+\epsilon)u$
          & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         
         (U)ConC$k$C  & Con$k$C~\cite{ge2008ConkC, liang2016ConkC} & \multicolumn{2}{c|}{(U)C$k$C~\cite{KhullerSussmanCkC}} & &\\
         & $6$ & $6$ & Nil & $18$ & Nil \\
        \hline
        
        (NU)ConC$k$C & Con$k$C~\cite{ge2008ConkC, liang2016ConkC} & \multicolumn{2}{c|}{(NU)C$k$C~\cite{AnCkC}} & &\\
        & $6$ &  $9$ & Nil & $24$ & Nil \\
         \hline
    \end{tabular}
\caption{Results corresponding to Theorems~\ref{thm_ConCFL} and~\ref{thm_ConCkC} based on current best approximation for the underlying problem. (U-Uniform, NU-Non-Uniform)}
    \label{tab_results1}
\end{table}





\begin{table}[]
    \centering
    \begin{tabular}{|c|c c|c c c|c|c|}
        \hline
         \textbf{Problem} & \multicolumn{2}{c|}{\textbf{Sub-problem 1}} & \multicolumn{3}{c|}{\textbf{Sub-problem 2}} &   \textbf{ Factor} & \textbf{Violation} \\ 
          & Problem  & Factor & Problem & Factor & Violation  & &  \\ 
         \hline
         (U)ConCFL  & ConFL~\cite{ConFLGrandoni2011} & $3.19$ & (U)CFL~\cite{Aggarwal} & $3$ & -  & $9.19$ & - \\
         \hline
         (NU)ConCFL  & ConFL~\cite{ConFLGrandoni2011} & $3.19$ & (NU)CFL~\cite{Bansal} & $5$ & -  &  $13.19$ & - \\
         \hline
         (U)ConC$k$M & ConFL~\cite{ConFLGrandoni2011} & $3.19$ & (U)C$k$M~\cite{ByrkaRybicki2015} & $ O(1/\epsilon)$ & $(1+\epsilon)u$ &  $O(1/\epsilon)$  & $(1+\epsilon)u$ \\
         \hline 
         (NU)ConC$k$M & ConFL~\cite{ConFLGrandoni2011} & $3.19$ & (NU)C$k$M~\cite{Demirci2016} & $O(1/\epsilon)$ & $(1+\epsilon)u$ &  $O(1/\epsilon)$  & $(1+\epsilon)u_i$ \\
         \hline 
         (U)ConC$k$FL & ConFL~\cite{ConFLGrandoni2011} & $3.19$ & (U)C$k$FL~\cite{capkmByrkaFRS2013} & $O(1/\epsilon^2)$ & $(2+\epsilon)u$
          & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         (U)ConC$k$C  & Con$k$C~\cite{ge2008ConkC, liang2016ConkC} & $6$ & (U)C$k$C~\cite{KhullerSussmanCkC} & $6$ & - & $18$ & - \\
        \hline
        (NU)ConC$k$C & Con$k$C~\cite{ge2008ConkC, liang2016ConkC} & $6$ & (NU)C$k$C~\cite{AnCkC} & $9$ & - & $24$ & -\\
         \hline
    \end{tabular}
\caption{Results corresponding to Theorems~\ref{thm_ConCFL} and~\ref{thm_ConCkC} based on current best approximation for the underlying problem. (U-Uniform, NU-Non-Uniform)}
    \label{tab_results1}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{|c|c c|c c c|c|c|}
    \hline
         \textbf{Problem} & \multicolumn{2}{c|}{\textbf{Sub-problem 1}} & \multicolumn{3}{c|}{\textbf{Sub-problem 2}} &   \textbf{ Factor} & \textbf{Violation} \\ 
          & Problem  & Factor & Problem & Factor & Violation & &  \\ 
         \hline
         (U)ConCPFL & ConPFL[This Paper] & $21.31$ & (U)CPFL[This Paper] & $5$ & - &  $31.32$ & - \\
         \hline
         (NU)ConCPFL & ConPFL[This Paper] & $21.31$ & (NU)CPFL[This Paper] & $5$ & - &  $31.32$ & - \\
         \hline
         (U)ConCP$k$M & ConPFL[This Paper] & $21.31$ & (U)CP$k$M~\cite{DabasCFLPO} & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ &  $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         (U)ConCP$k$FL & ConPFL[This Paper] & $21.31$ & (U)CP$k$FL~\cite{DabasCFLPO} & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ &  $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         ConPFL &  ConFL~\cite{ConFLGupta2001} & $10.66$ & \multicolumn{3}{c|}{-} & $21.32$ & -\\
        \hline
        (U)CPFL & \multicolumn{2}{c|}{-} & (NU)CFL[This paper] & $5$ & - & $5$ & - \\
         \hline
         (NU)CPFL &\multicolumn{2}{c|}{-} & (NU)CFL[This paper] & $5$ & - & $5$ & - \\
         \hline
    \end{tabular}
    \caption{Results corresponding to Theorems~\ref{thm_ConCPFL},~\ref{thm_ConPFL} and~\ref{thm_CPFL} based on current best approximation for the underlying problem. (U-Uniform, NU-Non-Uniform) }
    \label{tab_results3}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 2 (Factor, Violation)}  &\textbf{ Factor} & \textbf{Violation} \\ 
         \hline
         (U)\ConCPFL & (U)\CPFL($3$, Nil)~\cite{GuptaG14}) &  $27.32$ & Nil \\
         \hline
         (NU)\ConCPFL & (NU)\CPFL($5$, Nil)~\cite{GuptaG14} &  $31.32$ & Nil \\
         \hline
         (U)ConCPkM & (U)CPkM($O(1/\epsilon^2),(2+\epsilon)u$)~\cite{DabasCFLPO}) &  $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         (U)\ConCPkFL & (U)\CPkFL($O(1/\epsilon^2),(2+\epsilon)u$)~\cite{DabasCFLPO}) &  $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
    \end{tabular}
    \caption{Results corresponding to Theorem~\ref{thm_ConCPFL} based on current best approximation for the underlying problem. Sub-Problem 2 considered is \ConPFL for which we use $21.32$-factor approximation given in this paper. (U-Uniform, NU-Non-Uniform) }
    \label{tab_results3}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem }  &\textbf{ Factor}  \\ 
         \hline
        ConPFL & ConFL ($10.66$) ~\cite{ConFLGupta2001} & $21.32$\\
        \hline
        (U)CPFL & (NU)CFL ($5$)~[This paper] & $5$ \\
         \hline
         (NU)CPFL & (NU)CFL ($5$)~[This paper] & $5$ \\
         \hline
    \end{tabular}
\caption{Results corresponding to Theorem~\ref{thm_ConPFL} and~\ref{thm_CPFL} based on current best approximation for the underlying problem. (U-Uniform, NU-Non-Uniform) }
    \label{tab_results4}
\end{table}

==> extra.tex <==
Table~\ref{tab_results} summarises the results of this paper.
\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 1 (factor , Violation)} & \textbf{Sub-problem 2 (factor)} &\textbf{ Factor} & \textbf{Violation}  &
         \hline
         (U)\ConCFL  & (U)\CFL($3$~\cite{Aggarwal}) & \ConFL($3.19$~\cite{ConFLGrandoni2011}) & $9.19$ & Nil &
         \hline
         (NU)\ConCFL  & (NU)\CFL($5$~\cite{Bansal}) & \ConFL($3.19$~\cite{ConFLGrandoni2011}) & $13.19$ & Nil &
         \hline
         (U)\ConCkM & (U)\CkM($ O(1/\epsilon),(1+\epsilon)$~\cite{ByrkaRybicki2015}) & \ConFL($3.19$~\cite{ConFLGrandoni2011}) & O(1/\epsilon)  & $(1+\epsilon)u$ &
         \hline 
         (NU)\ConCkM & (NU)\CkM($ O(1/\epsilon) ,(1+\epsilon)$~\cite{Demirci2016}) & \ConFL($3.19$~\cite{ConFLGrandoni2011}) &O(1/\epsilon)  & $(1+\epsilon)u_i$ &
         \hline 
         (U)\ConCkFL & (U)\CkFL($O(1/\epsilon^2), (2+\epsilon)u$~\cite{capkmByrkaFRS2013}
         ) & \ConFL($3.19$~\cite{ConFLGrandoni2011}) & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ &
         \hline
         (U)\ConCPFL & (U)\CPFL($3$~\cite{GuptaG14}) & \ConPFL($21.32$~[this paper]) & $27.32$ & Nil &
         \hline
         (NU)\ConCPFL & (NU)\CPFL($5$~[this paper]) & \ConPFL($21.32$~[this paper]) & $31.32$ & Nil &
         \hline
    \end{tabular}
    \caption{First Constant Factor Approximations for variants of FL with capacity and connectivity constraints. (U-Uniform, NU-Non-Uniform)}
    \label{tab_results}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{| m{2cm} | m{10em} | m{10em} | m{1cm} | m{1.5cm} |}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 1 factor Violation} & \textbf{Sub-problem 2 factor} &\textbf{ Factor} & \textbf{Violation}   \\
         \hline
         (U)\ConCFL  & (U)CFL $3$~\cite{Aggarwal} Nil
         & \ConFL $3.19$~\cite{ConFLGrandoni2011} & $9.19$ & Nil  \\
         \hline
         (NU)\ConCFL  & (NU)\CFL $5$~\cite{Bansal} Nil & \ConFL $3.19$~\cite{ConFLGrandoni2011} & $13.19$ & Nil \\
         \hline
         (U)\ConCkM & (U)\CkM ($ O(1/\epsilon)~\cite{ByrkaRybicki2015})$) $(1+\epsilon)$  & \ConFL ($3.19$~\cite{ConFLGrandoni2011}) & O(1/\epsilon)  & $(1+\epsilon)u$ \\
         \hline
         (NU)\ConCkM & (NU)\CkM ($ O(1/\epsilon) ,(1+\epsilon)$~\cite{Demirci2016}) Nil & \ConFL ($3.19$~\cite{ConFLGrandoni2011}) &O(1/\epsilon)  & $(1+\epsilon)u_i$ \\
         \hline
         (U)\ConCkFL & (U)\CkFL ($O(1/\epsilon^2)~\cite{capkmByrkaFRS2013}
         )$ $(2+\epsilon)u$ & \ConFL ($3.19$~\cite{ConFLGrandoni2011}) & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
         (U)\ConCPFL & (U)\CPFL ($3$~\cite{GuptaG14}) Nil & \ConPFL ($21.32$~[this paper]) & $27.32$ & Nil \\
         \hline
         (NU)\ConCPFL & (NU)\CPFL($5$~[this paper]) & \ConPFL($21.32$~[this paper]) & $31.32$ & Nil \\
         \hline
    \end{tabular}
    \caption{First Constant Factor Approximations for variants of FL with capacity and connectivity constraints. (U-Uniform, NU-Non-Uniform)}
    \label{tab_results}
\end{table}


The problem of locating charging stations can be formulated as a facility location problem. {\em Facility Location Problem} (FL) is a well known and well studied problem in operations research and computer science~\cite{Shmoys,ChudakS03,Jain:2001,Byrka07,guha1999greedy,KPR,Chudak98,mahdian2001greedy,mahdian_1.52,charikar2005improved,arya,Zhang2007126,Li13}. In (uncapacitated) FL, we are given a set $\facilityset$ of facilities and a set $\cliset$ of clients.  A facility $i$ in $\facilityset$ has an associated {\em facility opening cost} $f_i$. $\dist{i}{j}$ denotes the cost of serving client $j$ from a facility $i$. We assume that the service cost is a metric.
%The distances between client $j$ and facility $i$, denoted by $\dist{i}{j}$ forms a metric.
The goal is to open $\facilityset' \subseteq \facilityset$ so as to minimise the sum of facility opening costs ({\em facility cost}) and the total {\em service cost} of serving all the clients from the opened facilities. In case of charging stations, the facilities are charging stations and the consumers are clients. Another closely related problem is $k$-Median problem ($k$M). In (uncapacitated) $k$M, we are given an upper bound $k$ ({\em cardinality constraint}) on the maximum number of facilities that can be opened in our solution and facility opening costs are $0$ for every facility. $k$-Facility Location is a common generalisation of FL and $k$M where in we have both the facility opening costs and the cardinality constraint. Yet another variant is, $k$-center problem ($k$C) where we wish to minimise the maximum distance of any client from the serving facility.


\subsection{Our Results}
Thought FL and its variants have been studied with capacities and connectivity separately, to the best of our knowledge, the common generalisations of FL/$k$M/$k$FL, where we have both connectivity and the capacity constraints have not been studied in the literature. We call these variants, {\em Connected Capacitated Facility Location Problem} (\ConCFL), {\em Connected Capacitated $k$-Median Problem} (\ConCkM) and, {\em Connected Capacitated Facility Location Problem} (\ConCkFL) and {\em Connected Capacitated $k$-Center} (ConC$k$C) respectively. \textcolor{red}{In this paper, we present \textcolor{blue}{first}
constant factor approximations for the problems by combining the solutions of the underlying problems (\CFL, \CkM, \CkFL) and \ConFL. For ConC$k$C, we combine C$k$C and Con$k$C. While combining the solutions, the violation in capacities/cardinality are preserved from the underlying problems}. To the best of our knowledge, no result is known for the problems with cardinality constraint and the only known result for ConCFL in the literature is by Friggstad~\etal~\cite{FriggstadConLUFL2016}. They gave a constant factor approximation for lower and (uniform) upper bounded ConFL violating both upper and lower bounds. \textcolor{blue}{We cannot get rid of the  violations in the upper bounds even when there are no lower bounds using their technique as they use LP rounding and the LP is known to have an unbounded integrality gap.} In this paper, we give the first true constant factor approximation for the problem and variants with non-uniform capacities. In particular, we present the following: 

\begin{theorem}
\label{thm_ConCFL}
Given an $\alpha$-factor approximation for CFL/C$k$M/C$k$FL/C$k$C with $\gamma$-factor violation in capacity/cardinality and a $\beta$-factor approximation for \ConFL/ConFL/ConFL/Con$k$C, 
a $(2\alpha+\beta)$-factor approximation for ConCFL/ConC$k$M/ConC$k$FL/ConC$k$C with $\gamma$-factor violation in capacity/cardinality respectively can be obtained in polynomial time.
\end{theorem}

We next consider the variant of the problem with penalties, called {\em Connected Prize-Collection Facility Location} (\ConPFL) and {\em Connected Prize-Collection $k$-Facility Location} (ConP$k$FL). {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. \PFL is a well studied problem in the literature~\cite{charikar2001algorithms, jain2003greedy, Wang2015penalties, xu2005lp, xu2009improved, LiDXX15, QiuWalter}. We study the connected and capacitated variants of \PFL.  In particular, we present the following:

\begin{theorem}
\label{thm_ConCPFL}
Given an $\alpha$-factor approximation for \CPFL/CP$k$M/\CPkFL with $\gamma$-factor violation in capacities and a $\beta$-factor approximation for \ConPFL, 
a $(2\alpha+\beta)$-approximation for \ConCPFL/\ConCP$k$M/\ConCPkFL with $\gamma$-factor violation in capacities can be obtained in polynomial time.
\end{theorem}

For ConPFL, we present the first constant ($21.32$) factor approximation by reducing the problem to ConFL using LP rounding techniques. In particular we present Theorem~\ref{thm_ConCPFL}. Note here, the underlying solution we have used is the one obtained using LP-rounding techniques. This is crucial and we can not use other (better approximation solutions) because of how we have performed the reduction.

\begin{theorem}
\label{thm_ConPFL}
Given a $\beta$-factor approximation for \ConFL (obtained using LP rounding techniques), a $2\beta$-factor approximation for \ConPFL can be obatined in polynomial time.
\end{theorem}


We present one simplified result for (non-uniform) \CPFL. Though there are results known in the literature for the problem with similar approximation guarantee ($5$-factor) by ~Gupta and Gupta~\cite{GuptaG14} using local search technique. Our result is interesting as it is much simpler and uses the underlying problem {\CFL} as black box without increasing the cost. Our factor will improve, if the factor for underlying problem (non-uniform CFL) can be improved in future. In particular, we present the following:

\begin{theorem}
\label{thm_CPFL}
Given an $\alpha$-factor approximation for (non-uniform) \CFL, an $\alpha$-factor approximation for \CPFL can be obtained in polynomial time.
\end{theorem}

We reduce an instance of ConPFL to an instance of ConFL using LP rounding techniques. We first solve a linear program for ConPFL problem. Next, we remove every client that was paying penalty to an extent of at least half in LP optimal by paying full penalty for these clients.  The remaining clients are served to an extent of at least half. We make a fractional feasible solution for ConFL problem with the remaining clients by increasing the assignments of the remaining clients. The opening of facilities and the connection variables are increased accordingly. The solution of ConFL along with the clients that paid penalty to full extent is our approximate solution for ConPFL. Note that the reduction does not work in presence of cardinality constraints because increasing the opening of facilities can violate the cardinality constraint by a factor of $2$.

In all the problems we reduce our problems to sub-problems in a way that connectivity constraints move to one sub problem and capacity constraint to another. Then we solve the underlying problems as black box. To combine the solution of the underlying problem, we open the facilities opened in the problem with capacity constraint and assign the clients as they were assigned in that solution. We are only left with connecting the opened facilities via a steiner tree. For connecting these facilities, we use the solution with connectivity constraint. The facilities in that solution are already connected. We connect these facilities to facilities opened in our solution via clients. In penalty version of the problem, some clients can be paying penalty and hence it might not be possible to connect the facilities within bounded cost. To handle this situation, we make all the clients pay penalty that were paying penalty in either of the solution. Now, every opened facility serves at least one client and this client is served in both the solutions.



%We reduce an instance of CPFL to an instance of CFL by creating dummy facilities with every client, that is, for every client we make a collocated dummy facility with capacity $1$. The facility opening cost of the facility is equal to the penalty cost of the respected collocated client. To make a feasible solution, we consider an optimal solution and open the dummy facilities if the collocated client was paying penalty in the optimal solution along with other opened facilities. Next, we solve the instance of CFL problem using any approximate algorithm for CFL problem as black-box. If any dummy facility is opened, we close it by making the collocated client pay penalty, thereby obtaining an approximate solution of CPFL problem. Note that the reduction does not work in presence of the cardinality constraint because the number of opened facilities in the feasible solution will increase.

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 2 (Factor, Violation)}  &\textbf{ Factor} & \textbf{Violation} \\ 
         \hline
         (U)\ConCFL  & (U)\CFL ($3$, Nil) ~\cite{Aggarwal}  & $9.19$ & Nil \\
         \hline
         (NU)\ConCFL  & (NU)\CFL($5$, Nil) ~\cite{Bansal} &  $13.19$ & Nil \\
         \hline
         (U)\ConCkM & (U)\CkM($ O(1/\epsilon),(1+\epsilon)u$)~\cite{ByrkaRybicki2015} &  $O(1/\epsilon)$  & $(1+\epsilon)u$ \\
         \hline 
         (NU)\ConCkM & (NU)\CkM($ O(1/\epsilon) ,(1+\epsilon)u$)~\cite{Demirci2016} &  $O(1/\epsilon)$  & $(1+\epsilon)u_i$ \\
         \hline 
         (U)\ConCkFL & (U)\CkFL($O(1/\epsilon^2), (2+\epsilon)u)$~\cite{capkmByrkaFRS2013}
          & $O(1/\epsilon^2)$ & $(2+\epsilon)u$ \\
         \hline
    \end{tabular}
\caption{Results corresponding to Theorem~\ref{thm_ConCFL} based on current best approximation for the underlying problem. Sub-Problem 1 considered is \ConFL for which we use $3.19$-factor approximation of~\cite{ConFLGrandoni2011}). (U-Uniform, NU-Non-Uniform) }
    \label{tab_results1}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem 1 (Factor)} & \textbf{Sub-problem 2 (Factor)} &\textbf{ Factor}  \\ 
         \hline
        (U)ConC$k$C  & Con$k$C ($6$) ~\cite{ge2008ConkC, liang2016ConkC} & (U)C$k$C ($6$)~\cite{KhullerSussmanCkC} & $18$ \\
        \hline
        (NU)ConC$k$C& Con$k$C ($6$) ~\cite{ge2008ConkC, liang2016ConkC} & (NU)C$k$C  ($9$)~\cite{AnCkC} & $24$\\
         \hline
    \end{tabular}
\caption{Results corresponding to Theorem~\ref{thm_ConCkC} based on current best approximation for the underlying problem. (U-Uniform, NU-Non-Uniform) }
    \label{tab_results2}
\end{table}




==> old_intro.tex <==
\section{intro}

******************** old intro ********************
In some applications, there is an upper bound $u_i$ on the number of clients an opened facility $i$ can serve. 
\textcolor{red}{Do we need uniform anywhere?} The capacities are called uniform if $u_i$ is same for all $i$ in $\facilityset$.
\textcolor{red}{ If we are dealing with non-uniform then we don't need to say it explicitly...that is default....SO delete...
We will be dealing with general/non-uniform capacities in this paper.}

In some applications, it is important for the opened facilities to be connected to each other. For example, consider a telecommunication network model with a {\em central core} consisting of interconnected nodes and there is a set of {\em end nodes} that want to communicate with each other. Each core node (facility) has a switch cost and connecting central nodes to each other incurs some connection cost.  The goal is to select a subset of core nodes, connect these nodes to each other and end nodes (clients) to one of the selected core nodes so as to design a network of minimum cost. Such a variant of FL is called {\em Connected Facility Location Problem} (ConFL). ConFL is same as FL except we are also given distance $\concost{e}$ for every edge $e=(i_1, i_2)$ where $i_1,i_2 \in \facilityset$. %In a telecommunication network, the parameter $M$ reflects per unit cost of connection. 
The connectivity of the opened facilities is captured by a {\em Steiner tree} $T$, i.e., a tree connecting opened facilities but may consist of non-facility (client) nodes. %The total cost of interconnecting the facilities is $M$ times the cost of the steiner tree $T$. 
We call this cost the {\em connection cost}. We aim to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and the connection cost. ConFL is studied in the literature~\cite{ConFLGupta2001, ConFLGupta2004, ConFLSwamy2004,ConFLChwa2009,ConFLEisenbrand2010,ConFLGrandoni2011} and the current best approximation is due to Grandoni and Rothvob~\cite{ConFLGrandoni2011}. They used sampling techniques to give a $3.19$-factor approximation for the problem. Similar to CFL, variants of ConFL where we have cardinlity constraint have been studied in the literature, namely {\em Connected $k$-Median Problem} (\ConkM) and {\em Connected $k$-Facility Location Problem} (\ConkFL). The current best factor approximations ($6.98$) for \ConkM and \ConkFL are due to Eisenbrand~\etal~\cite{ConFLEisenbrand2010}.

\textcolor{red}{Though FL/$k$M/$k$FL have been studied with capacities and connectivity separately, to the best of our knowledge, their common generalisations where in we have both connectivity and the capacity constraints have not been studied earlier.  We call these variants, {\em Connected Capacitated Facility Location Problem} (\ConCFL), {\em Connected Capacitated $k$-Median Problem} (\ConCkM) and, {\em Connected Capacitated Facility Location Problem} (\ConCkFL) respectively.  Applications of these generalisations can be found in real life. In our example of telecommunication networks, as the switches have a limited number of slots, there is a natural cap on the maximum number of end nodes that can be connected to a core node. In this paper, we present \textcolor{blue}{first}
constant factor approximations for the problems by combining the solutions of the capacitated variants of the underlying problems (\CFL, \CkM, \CkFL) and \ConFL .
The violations in capacities/cardinality, if any, in the solutions of the underlying problems, are preserved. For \ConCkM and \ConCkFL, we present first approximations and for \ConCFL, our result is the first true approximation. To the best of our knowledge, the only result known for ConCFL is by Friggstad~\etal~\cite{FriggstadConLUFL2016}. They gave a constant factor approximation for lower and (uniform) upper bounded ConFL violating both the upper as well as the lower bounds.
{We cannot get rid of the  violations in the upper bounds even when there are no lower bounds using their technique as they use LP rounding and the LP is known to have an unbounded integrality gap.}
In this paper, we give the first true constant $(13.19)$-factor approximation for the problem using a true approximation for the CFL problem. In particular, we present the following: 
 }

Thought FL and its variants have been studied with capacities and connectivity separately, to the best of our knowledge, the common generalisations of FL/$k$M/$k$FL, where we have both connectivity and the capacity constraints have not been studied in the literature. We call these variants, {\em Connected Capacitated Facility Location Problem} (\ConCFL), {\em Connected Capacitated $k$-Median Problem} (\ConCkM) and, {\em Connected Capacitated Facility Location Problem} (\ConCkFL) respectively. The problems are same as \ConFL/\ConkM/\ConkFL except every facility $i$ can serve at most $u_i$ number of clients. \textcolor{red}{In this paper, we present \textcolor{blue}{first}
constant factor approximations for the problems by combining the solutions of the underlying problems (\CFL, \CkM, \CkFL) and \ConFL .
\textcolor{blue}{
The violations in capacities/cardinality, if any, in the solutions of the underlying problems, are preserved. For \ConCkM and \ConCkFL, we present first approximations and for \ConCFL, our result is the first true approximation.}
While combining the solutions, the violation in capacities/cardinality are preserved from the underlying problems}.
\st{
We first present our technique for \ConCFL by combining the solutions of \CFL and \ConFL and then extend these results to other variants.} To the best of our knowledge, the only known result for ConCFL in the literature is by Friggstad~\etal~\cite{FriggstadConLUFL2016}. They gave a constant factor approximation for lower and (uniform) upper bounded ConFL violating both upper and lower bounds.% A constant factor approximation for ConCFL with constant factor violation in capacities when the capacities are uniform follows as a special case of their problem. 
\st{
Firstly, their result holds only for uniform capacities.
Secondly, they violate the capacities.}
\textcolor{blue}{We cannot get rid of the  violations in the upper bounds even when there are no lower bounds using their technique as they use LP rounding and the LP is known to have an unbounded integrality gap.}
Their result can not be extended to get rid of violation in upper bounds even when there are no lower bounds as they use LP rounding techniques and the LP is known to have an unbounded integrality gap. % Finally, their factor is dependent on.... which can be large for small violation in capacities. 
In this paper, we give the first true constant $(13.19)$-factor approximation for the problem with non-uniform capacities. In particular, we present the following: 

\begin{theorem}
\label{thm_ConCFL}
Given an $\alpha$-factor approximation for \CFL/\CkM/\CkFL with $\gamma$-factor violation in capacity/cardinality and a $\beta$-factor approximation for \ConFL, 
a $(2\alpha+\beta)$-factor approximation for \ConCFL/\ConCkM/\ConCkFL respecting the violations,
%with $\gamma$-factor violation in capacity/cardinality respectively
can be obtained in polynomial time.
\end{theorem}

%The technique presented in our paper is very flexible as our factor can be improved without any change in the algorithm if, in future, the factors of the underlying problems improve. Also, the ideas extends easily to other variants of the problems. We get similar results for \ConCkM and \ConCkFL as mentioned in Theorem~\ref{thm_ConkM} and Theorem~\ref{thm_ConCkFL} respectively. To the best of our knowledge, these are the first approximations for the problems.

%\begin{theorem}
%\label{thm_ConkM}
%Given an $\alpha$-factor approximation for \CkM with $\gamma$ factor violation in capacities and a $\beta$-factor approximation for \ConFL, a $(2\alpha+\beta)$-factor approximation for \ConCkM with $\gamma$-factor violation in capacities can be obtained in polynomial time.
%\end{theorem}

%\begin{theorem}
%\label{thm_ConCkFL}
%Given an $\alpha$-factor approximation for \CkFL with $\gamma$ factor violation in capacities and a $\beta$-factor approximation for \ConFL, a $(2\alpha+\beta)$-factor approximation for \ConCkFL with $\gamma$-factor violation in capacities by $\gamma$-factor can be obtained in polynomial time.
%\end{theorem}

\textcolor{red}{ I am here..ng...are we not studying PkM and PkFL?
We next consider another variant of facility location problem, called {\em Connected Prize-Collection Facility Location} (\ConPFL). In the above formulations of the problem (say in telecommunication network), a few distant clients can affect the cost of the solution disproportionately. {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. \PFL is a well studied problem in the literature~\cite{charikar2001algorithms, jain2003greedy, Wang2015penalties, xu2005lp, xu2009improved, LiDXX15, QiuWalter}. We study the connected variant of \PFL. The two underlying problems here are \PFL and \ConFL and it is tempting to use combination of the two problems to obtain the solution. However, the combination technique does not extend to this variant of the problem because it is difficult to reduce \ConPFL to \ConFL directly within constant cost bounds. To handle this problem, we take help from LP-rounding techniques. We present the first constant ($21.31$)-factor approximation for the problem by using LP rounding technique followed by reduction to \ConFL.  In particular, we present the following:}



We next study another variant of connected facility location problem, called {\em Connected Prize-Collection Facility Location} (\ConPFL). In the above formulations of the problem (say in telecommunication network), a few distant clients can affect the cost of the solution disproportionately. {\em Prize-Collection Facility Location Problem} (PFL) is a generalization of the (uncapacitated) FL in which any client $j$ may be left unserved by paying a penalty $p_j$. Another way to think about it is that every client has a prize that can only be collected if it is served. The goal now is to open $\facilityset' \subseteq \facilityset$ so as to minimise the total of facility cost, service cost and {\em penalty cost}, which is the sum of all the penalties paid in the solution. Note that, in penalty version of the problem, service cost represents the total cost of servicing all the clients that were not paying penalty. \PFL is a well studied problem in the literature~\cite{charikar2001algorithms, jain2003greedy, Wang2015penalties, xu2005lp, xu2009improved, LiDXX15, QiuWalter}. We study the connected variant of \PFL. The two underlying problems here are \PFL and \ConFL and it is tempting to use combination of the two problems to obtain the solution. However, the combination technique does not extend to this variant of the problem because it is difficult to reduce \ConPFL to \ConFL directly within constant cost bounds. To handle this problem, we take help from LP-rounding techniques. We present the first constant ($21.31$)-factor approximation for the problem by using LP rounding technique followed by reduction to \ConFL.  In particular, we present the following:

\begin{theorem}
\label{thm_ConPFL}
Given a $\beta$-factor approximation for \ConFL (obtained using LP rounding techniques), a $2\beta$-factor approximation for \ConPFL can be obatined in polynomial time.
\end{theorem}


Finally, we consider the most common generalisation of the problems studied in the paper, that is, we combine capacities, connectivity and penalties in facility location problem. We call the problem as {\em Connected Capacitated Prize-Collecting Facility Location Problem} (\ConCPFL). We extend the ideas of combination technique to present the first constant ($31.31$) factor approximation for the problem with general capacities. The two underlying problems considered are {Capacitated Prize-Collecting Facility Location Problem} (\CPFL) and  {Connected Prize-Collecting Facility Location Problem} (\ConPFL). The idea extends to the problem with cardinality constraint as well, that is, to {\em Connected Capacitated Prize-Collecting $k$-Facility Location Problem}(\ConCPkFL).  In particular, we present the following:

\begin{theorem}
\label{thm_ConCPFL}
Given an $\alpha$-factor approximation for \CPFL/\CPkFL with $\gamma$-factor violation in capacities and a $\beta$-factor approximation for \ConPFL, 
a $(2\alpha+\beta)$-approximation for \ConCPFL/\ConCPkFL with $\gamma$-factor violation in capacities can be obtained in polynomial time.
\end{theorem}

Table~\ref{tab_results1}, ~\ref{tab_results2} and ~\ref{tab_results3} summarises the results of this paper. 


\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
         \textbf{Problem} & \textbf{Sub-problem(Factor)}  &\textbf{ Factor}  \\ 
         \hline
         \ConPFL & \ConFL (10.66) ~\cite{ConFLGupta2001} & $21.32$ \\
         \hline
  \end{tabular}
    \caption{Approximations for variant of FL with connectivity and penalty.}
    \label{tab_results2}
\end{table}  


\subsection{Additional Results}
We present one simplified result for (non-uniform) \CPFL. Though there are results known in the literature for the problem with similar approximation guarantee ($5$-factor) by ~Gupta and Gupta~\cite{GuptaG14} using local search technique. Our result is interesting as it is much simpler and uses the underlying problem {\CFL} as black box without increasing the cost. Our factor will improve, if the factor for underlying problem (non-uniform CFL) can be improved in future. In particular, we present the following:

\begin{theorem}
\label{thm_CPFL}
Given an $\alpha$-factor approximation for (non-uniform) \CFL, an $\alpha$-factor approximation for \CPFL can be obtained in polynomial time.
\end{theorem}

==> variants.tex <==
\subsection{Extending results to other variants}
\label{variants}
